Classification is a Strong Baseline for Deep Metric Learning

Deep metric learning aims to learn a function mapping image pixels to embedding feature vectors that model the similarity between images. Two major applications of metric learning are content-based image retrieval and face verification. For the retrieval tasks, the majority of current state-of-the-art (SOTA) approaches are triplet-based non-parametric training. For the face verification tasks, however, recent SOTA approaches have adopted classification-based parametric training. In this paper, we look into the effectiveness of classification based approaches on image retrieval datasets. We evaluate on several standard retrieval datasets such as CAR-196, CUB-200-2011, Stanford Online Product, and In-Shop datasets for image retrieval and clustering, and establish that our classification-based approach is competitive across different feature dimensions and base feature networks. We further provide insights into the performance effects of subsampling classes for scalable classification-based training, and the effects of binarization, enabling efficient storage and computation for practical applications.

==> metric_learning.tex <==
\section{Classification as Metric Learning}
\label{sec:cls_metric_learning}

In this section, we will prove that \textbf{removing bias} and \textbf{L2-normalizing} inputs and weights before the final softmax cross-entropy layer make classification a variant of proxy-based metric learning. We first examine the Neighborhood Component Analysis (NCA) Loss used as the surrogate loss for ranking in \cite{nofusslearning}. With the set of dissimilar images denoted as $Z$ and distance between embeddings of images $x, y$ as $d(x, y)$:
\begin{equation}\label{eq:ncaloss}
    L_{\text{NCA}}(x, y, Z) = -\log\left(\frac{\exp(-d(x,y))}{\sum_{z \in Z} \exp(-d(x, z))}\right)
\end{equation}
We argue that by excluding the positive term $exp(-d(x,y))$, the proxy-NCA loss does not have the probabilistic meaning as proposed in original NCA paper\cite{nca}. The softmax cross-entropy loss (softmax loss) used in standard classification task, on the other hand, which is more similar to NCA loss in spirit, also tries to make $x$ closer to $y$ than any $z \in Z$. 
\begin{multline}\label{eq:celoss}
    L_{\text{cls}}(x, y, Z) = \\
    -\log\left(\frac{\exp(-d(x,y))}{\exp(-d(x,y)) + \sum_{z \in Z} \exp(-d(x, z))}\right)
\end{multline}
With the static proxy assignment and the choice of distance function being the \textbf{cosine distance}:
\begin{equation}
\begin{split}
    d(x, y) = 1 - x^Ty \\
\end{split}
\end{equation}
The proxy-classification loss can then be expressed as standard softmax loss when input and weights are L2-normed:
\begin{multline}\label{eq:proxy_cls_loss}
    L_{\text{cls}}(x, p_y, p_Z) \\
    = -\log\left(\frac{\exp(-(1 - x^Tp_y))}{\sum_{p_z \in (p_Z \cup p_y)} \exp(-(1 - x^Tp_z))}\right) \\
    = -\log\left(\frac{\exp(x^Tp_y))}{\sum_{p_z \in (p_Z \cup p_y)} \exp(x^Tp_z))}\right)
\end{multline}
% Try to derive the loss bound
By using the network's penultimate layer's normalized output as the embedding, and the normalized weights of the last fully-connected layer as the proxies, we show that standard classifier training \textbf{without bias} in the last layer is just a variant of proxy-based metric learning. We refer this modified softmax loss as \textbf{normalized softmax loss}. This explains the strong baseline observed by simply using the activations of the network pre-trained on a classification task such as ImageNet\cite{imagenet_cvpr09}. We can also leverage the vast body of literature on the tricks for optimizing classification task training and performance.

